Principal Surface Fault Rupture Hazard: Moving Beyond Aggregate Displacement Metrics

Structures crossing active faults are subjected to permanent ground deformation that can impose severe demands on infrastructure. Although probabilistic fault displacement hazard analysis (PFDHA) has advanced considerably, existing principal fault displacement models use aggregate displacement, implicitly assuming that overlapping rupture strands contribute simultaneously to site demand. This assumption is suitable for regional hazard characterization but does not represent finite structural dimensions, where only a subset of ruptures may intersect a structure. This study presents a probabilistic framework that reformulates aggregate principal displacement into a rupture-level representation for infrastructure-specific hazard assessment. Using the Fault Displacement Hazard Initiative (FDHI) database of 75 surface-rupturing earthquakes, principal rupture strands are reconstructed from mapped rupture geometries and displacement observations using event- and segment-based coordinate systems. The framework models three quantities: (1) the number of overlapping principal ruptures, (2) partitioning of aggregate displacement among individual rupture strands while preserving the aggregate displacement budget, and (3) the spatial distribution of rupture strands relative to the primary fault trace. These components are integrated into a generalized PFDHA formulation accounting for earthquake magnitude, style of faulting, rupture curvature, structural footprint, and fault-trace location uncertainty. Benchmark fault-crossing applications demonstrate the framework's ability to estimate the probability that individual rupture strands intersect a structure and the associated displacement demand. The framework provides a physically consistent extension of aggregate-based models and a basis for infrastructure-specific PFDHA that explicitly accounts for rupture geometry and finite crossing dimensions.

==> scrap.tex <==
% ---------------------------------------------------------

In parallel, \cite{wesnousky2008displacement} compiled surface rupture maps and coseismic slip observations from historical earthquakes and showed that these data provide a statistical basis for describing along-strike variability of surface displacement and for constraining rupture endpoints. The observations support the existence of a finite process zone at rupture terminations, within which stress changes may promote slip on adjacent faults, emphasizing the role of rupture geometry and fault complexity in controlling surface displacement patterns and reinforcing that surface displacement should be treated as spatially variable along rupture traces rather than uniform.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/Introduction/principal and distributed displacement (ypung et al.).pdf}
%     \caption{Principal and distributed faulting pattern (adopted from Young et al. [])} 
%     \label{fig: Principal and distributed displacement}
% \end{figure}

% ---------------------------------------------------------


Building directly on this foundation, \cite{lavrentiadis2025fault} developed a probabilistic fault displacement model that explicitly represents rupture-level variability and partitions total surface displacement into principal and distributed components. Using standardized FDHI observations from global surface-rupturing earthquakes, they modeled aggregate displacement as a function of earthquake magnitude and normalized along-strike position, and then decomposed it into principal and distributed slip using statistically consistent formulations, enabling exceedance-based hazard calculations for both aggregate and component displacements. In parallel, \cite{lavrentiadis2025seismologically} developed a seismologically consistent surface rupture length (SRL) model that distinguishes between unbounded and width-limited ruptures and evaluated its performance through comparisons with widely used SRL models, including \cite{wells1994new}, \cite{wesnousky2008displacement}, \cite{leonard2010earthquake}, \cite{leonard2014self}, and \cite{wells2015improved}, showing improved fit particularly for large-magnitude, width-limited events while maintaining consistency at smaller magnitudes. Most recently, \cite{sarmiento2025comparisons} performed a comprehensive comparison of updated FDHI-based fault displacement models using a standardized dataset of 75 global earthquakes and evaluated LA23 (\cite{lavrentiadis2025fault}), MEA24 (\cite{moss2025new}), KEA24 (\cite{kuehn2025fault}), and CEA25 (\cite{chiou2025fault}), noting that these models differ in statistical formulation and treatment of magnitude scaling and along-strike variability while generally achieving improved agreement with observed principal and aggregate displacement data compared to earlier approaches.
Collectively, these studies define the empirical and probabilistic foundation of PFDHA, showing a clear evolution from magnitude-based rupture scaling and post-event field observations toward standardized datasets and rupture-informed probabilistic models that can generate hazard metrics. At the same time, across much of this development, displacement is still frequently represented through aggregate displacement, where aggregate here refers to the total surface offset of principal or distributed displacement, as illustrated in Figure \ref{fig: Aggregate vs principal displacement} for principal displacement. Moreover, although recent FDHI-based models represent along-strike variability more systematically, geometric complexity, such as rupture curvature, is not considered. This leaves a gap between increasingly sophisticated statistical formulations and the physics-informed geometric controls that govern how displacement is partitioned and expressed spatially at the surface, especially for infrastructure that intersects. These limitations motivate the need for more accurate, physics-informed PFDHA methods that can move design practice beyond reliance on engineering judgment and toward more accurate displacement hazard assessments.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/Framework/Agg vs principal.pdf}
    \caption{Aggregate principal and principal displacement} 
    \label{fig: Aggregate vs principal displacement}
\end{figure}
